Intuitionistic Justification Logic, Semantically

Justification logics are explicit versions of modal logic. In the classical setting, this means boxes are refined with explicit proof terms and interact with each other through proof operations. This exercise was extended to intuitionistic modal logic with native diamonds. In this setting, diamonds are refined to satisfier terms and come equipped with additional operations. Justification logic enjoys a connection to its corresponding modal logic through a realisation theorem. In the classical setting, this is achieved through either proof-theoretic or semantic methodology. So far, intuitionistic justification logic with satisfiers has only been presented syntactically with a proof-theoretic realisation theorem. We present two classes of semantics for intuitionistic justification logic with soundness and completeness results: basic modular models, which extend possible world semantics for intuitionistic propositional logic; modular models which contain Kripke-style machinery to promote "backwards compatibility" to modal logic. Using modular models, we present a realisation theorem to establish a connection between intuitionistic justification logic and its corresponding intuitionistic modal logic.

==> eptcsdata.tex <==
\providecommand{\firstpage}{603}
\providecommand{\publicationstatus}{M.~B\'ilkov\'a, M.~Gattinger, I.~van~der~Giessen, M.~Girlando, Y.~Wang (Eds.):\\
Advances in Modal Logic 2026 (AiML 2026)\\
EPTCS 447, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.447.34}{10.4204/EPTCS.447.34}}
\pdfoutput=1

